Reduced I/O Latency with Futures

Task parallelism research has traditionally focused on optimizing computation-intensive applications. Due to the proliferation of commodity parallel processors, there has been recent interest in supporting interactive applications. Such interactive applications frequently rely on I/O operations that may incur significant latency. In order to increase performance, when a particular thread of control is blocked on an I/O operation, ideally we would like to hide this latency by using the processing resources to do other ready work instead of blocking or spin waiting on this I/O. There has been limited prior work on hiding this latency and only one result that provides a theoretical bound for interactive applications that use I/Os. In this work, we propose a method for hiding the latency of I/O operations by using the futures abstraction. We provide a theoretical analysis of our algorithm that shows our algorithm provides better execution time guarantees than prior work. We also implemented the algorithm in a practically efficient prototype library that runs on top of the Cilk-F runtime, a runtime system that supports futures within the context of the Cilk Plus language, and performed experiments that demonstrate the efficiency of our implementation.

==> Makefile <==
# Standard Makefile for compiling LaTeX documents in the Supertech
# group.

# DOC=$(shell basename $(CURDIR))
DOC=futureIO

# This line is intentionally blank.

TARGETS=$(patsubst %,%.pdf,$(DOC))

OTHERS = Makefile supertech-acm.sty papers.bib # plain-url.bst

DEPS_DIR = .deps

INCLUDE_DIR=.

LATEXMK = TEXINPUTS=$(INCLUDE_DIR)/: BIBINPUTS=$(INCLUDE_DIR)/: BSTINPUTS=$(INCLUDE_DIR)/: latexmk
LATEXMK_FLAGS = -pdflatex="pdflatex --shell-escape %O %S" -pdf -dvi- -ps- -recorder -M -MP \
                  -e 'show_cus_dep();' \

default: pdf
.PHONY:  pdf default all remake clean allclean

all: $(TARGETS)

-include $(DEPS_DIR)/$(DOC).pdfP

ifneq (,$(findstring B,$(MAKEFLAGS)))
LATEXMK_FLAGS += -gg
endif

$(DEPS_DIR) :
	if [ ! -d $(DEPS_DIR) ]; then mkdir $@; fi

$(DOC).pdf : $(OTHERS)

###########################################################################
## Make targets for cleaning

clean%:
	rm -f $*.aux $*.ps $*.pdf $*.dvi $*.bbl $*.blg $*.tmp $*.lof $*.log $*.toc $*.out $*.fls $*.fdb_latexmk $(DEPS_DIR)/$*.pdfP *~ *.tex.bak

clean: clean$(DOC)

allclean:
	rm -f *.aux *.dvi *.bbl *.blg *.tmp *.lof *.log *.toc *.out *.fls *.fdb_latexmk $(DEPS_DIR)/*.pdfP $(DOC).pdf *~



###########################################################################
## Make targets for document

pdf : $(DOC).pdf

%.pdf : %.tex $(OTHERS)
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) $(LATEXMK_FLAGS) -MF $(DEPS_DIR)/$@P $<
	if [ -e $@ ]; then touch $@; fi

# Some nonsense that latexmk doesn't understand with minted can be fixed by telling that these rules are easy.
%.w18 %.out.pyg %.aex: %.tex
	@echo > /dev/null
# remake :
# 	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
# 	$(LATEXMK) -g -deps-out=$(DEPS_DIR)/$(DOC).pdfP $(DOC).tex
# 	if [ -e $(DOC).pdf ]; then touch $(DOC).pdf; fi


==> cut.tex <==
%% eval 
%%=======================================================================

ere largely due to the ability of
\SYS to hide a majority of the latency, even when executing on a single core.
Figure \ref{fig:overhead} shows the execution times of \benchName using \SYS
with latencies ranging from 1 to 500 ms and using Cilk Plus without any I/O
latency (\textit{ideal}), as well as the speedups compared to $T_1$ of the
\textit{ideal} row. The ideal case would be for the timestamps and speedups to
all be equal to that of \textit{ideal}. Although \SYS never quite matches
\textit{ideal}, it gets fairly close in some situations. As can be seen from
the table, however, we still see a fair amount of performance degradation from
increasing I/O latencies. We manage to hide a lot of the latency, but even so
a small amount of that latency appears in our results.

%% system
%%=======================================================================

I/O operations whose file descriptors that are not ready can be added to an
\IOT's individual \epoll set, and sleep until one or more file descriptors can
accept I/O operations, eliminating the need to manually wake up and check the
status of each file. Although this allows the \epoll facility to solve the CPU
sharing problem for monitoring file descriptors, the \commQ would still need
to be monitored for updates as well. This could again be achieved by providing
a timeout when sleeping using the \epoll handle, but this would mean \epoll
has not solved the problem. Linux provides, however, an event wait/notify
mechanism called \eventfdCite. The \eventfd mechanism is used to create a file
descriptor that can be written to by the normal worker, and read by the \IOW.
This file descriptor can be opened with semaphore-like semantics, in which
writes will increment a backing counter and reads will decrement the same
counter. When used with \epoll, a write to an \eventfd file descriptor will
cause the \IOT to wake whenever the backing counter is incremented from 0 to
1. By writing to an \eventfd file descriptor associated with a \commQ whenever
an I/O operation is enqueued, and by symmetrically reading from the same file
descriptor whenever an operation is dequeued, \epoll can also be used to
monitor the state of the \commQ. We use this combination of \eventfd and
\epoll in order to allow the \IOTNoSpace s to sleep whenever there are neither
any file descriptors it can perform I/O on nor any I/O operations pending in
the \commQ.

%%=======================================================================

Linux's \epoll can be used to monitor a set of file descriptors (an \epoll
set) and determine when a specified I/O operation can be performed.  This set
of file descriptors is associated with an \epoll instance, and there can be
many \epoll instances with differing \epoll sets in a program.  Adding a file
to be monitored is fast, and is an $O(lgn)$ operation, where $n$ is the number
of file descriptors currently in the \epoll set. Determining whether to sleep
or continue processing when checking the status of an \epoll set, however, is
an $O(1)$ operation, since adding a file descriptor to the \epoll set
registers a callback with the file's underlying system driver. This callback
will move the file into a ready list and wake the monitoring thread when I/O
on that file becomes possible.

%%=======================================================================

Once an \IOW empties its \commQ, it needs to monitor the file descriptors of
any I/O operations that could not be completed in order to detect when the
files become ready for the operation. One solution would be to have the \IOT
sleep and periodically wake up to check the status of all of files for which
there are pending operations (as well as the status of the \commQ). This
scheme would cause the \IOT to steal cycles from the regular worker,
potentially interrupting progress into the computation when there is nothing
for the \IOW to do.

%%=======================================================================

When an \IOW runs, it dequeues items from the \commQ and attempts to perform
an I/O operation as soon as it is received.  Whenever the \IOW completes one
of the I/O operations, it performs a \putF on the corresponding \ioF handle.
If an I/O operation cannot be completed immediately (e.g., the next package
has not arrived on the network channel yet), however, the request is put aside
to be processed later when the I/O device becomes ready (has more input to be
consumed).  

In order to describe the actual mechanism, we need to review how I/O operates
on Linux.  On Linux, obtaining input from a file descriptor is effectively
copying data from the corresponding device into memory (e.g., the $buf$ in the
example).  If the device is not ready to be read (e.g., the next package has
not arrived on the network channel yet) the system call \sysRead will block.
One could make the system call with the correct flag so that the system call
would simply return (with a return value indicating input not ready) instead
of blocking.  However, that means the \IOW needs to wake up periodically and
poll via the system calls. 

%%=======================================================================

\SYS is based on the Cilk-F \cite{SingerXuLe19} runtime, which extends Intel
Cilk Plus \cite{IntelCilkPlus13,IntelCilkPlusLangSpec13} to support scheduling
futures. Cilk-F implements a \textit{\textbf{proactive work-stealing
scheduler}}, which behaves the same as a classic parsimonious work-stealing
scheduler until a task must suspend when synchronizing with a \getF call on a
future handle. In proactive work stealing, if a worker's deque is non-empty
when such a synchronization attempt is made, the worker will suspend the deque
(though the deque will remain a steal target), create a new deque, and become
a thief to steal work. Since it is possible to have many concurrently
suspended deques, the runtime takes extra precautions to ensure that the
suspended deques are roughly balanced among the workers by selecting two
random workers and storing the suspended deque with the worker with the fewest
suspended deques. As \SYS extends Cilk-F, this behavior is present in \SYS as
well.

%%=======================================================================

\begin{algorithm}
%\resumenumbering
\footnotesize

% Function def 
\SetKwProg{Fn}{Function}{}{end}
% Functions on future handles 
\SetKwFunction{GetFuture}{\getFNoSpace}
\SetKwFunction{PutFuture}{\putFNoSpace}
% I/O Functions
\SetKwFunction{CilkWrite}{\cilkWriteNoSpace}
\SetKwFunction{CilkRead}{\cilkReadNoSpace}
\SetKwFunction{DistMapRed}{\distMapReduce}
\SetKwFunction{OpenConnection}{openConnection}

% Define new keywords
\SetKw{Break}{break}
\SetKw{Continue}{continue}
\SetKw{Spawn}{\spawn}
\SetKw{Sync}{\sync}
\SetKw{NBYTES}{NBYTES}

% Styling
\SetInd{0.5em}{0.5em}
\SetNlSkip{0.5em}
\SetKwComment{tcp}{/\hspace{-0.2em}/}{\hspace{0.5em}}

\Fn{\DistMapRed{$f$, $g$, $id$, $lo$, $hi$}} {
    $n \gets hi - lo$\;

    \lIf{n = 0}{\Return $id$}
    \ElseIf{n = 1}{
        char inBuf[\NBYTES]; \tcp{The buffer the data will be read into.}

        $connectionFd \gets$ \OpenConnection{$lo$}; 
                        \tcp{Open a file descriptor.}
                        \label{mr:connect}
        $\ioF fut \gets$ \cilkReadNoSpace{$connectionFd$, $inBuf$, \NBYTES};
                        \label{mr:read}
        \GetFuture{$fut$};

        \Return f($inBuf$);
    } \Else {
        $mid \gets (lo + hi) / 2$;

        $r1 \gets$ \Spawn \DistMapRed{$f$, $g$, $id$, $lo$, $mid$}\;

        $r2 \gets$ \DistMapRed{$f$, $g$, $id$, $mid$, $hi$}\;

        \Sync;

        \Return g($r1$, $r2$); \label{mr:g}
}
}
%FIXME: cite their paper
\caption{Muller and Acar's \cite{MullerAc16} distributed map and reduce using \SYS}
\label{fig:example}
\end{algorithm}

%% intro
%%=======================================================================

As far as we know, only one prior work exists that directly tackles the issue
of provably efficient scheduling of task parallel code with I/Os.  Muller and
Acar~\cite{MullerAc16} present a cost model and its corresponding scheduling
theory for reasoning about latency incurring operations (such as I/Os) in task
parallel programs.  Typically, a task parallel computation is modeled as a
\defn{directed acyclic graph}, or \defn{dag}~\cite{BlumofeLe99}, where each
node represents a \defn{strand}, a sequence of instructions containing no
parallel keywords, and the edges represents control dependencies between
strands (i.e., an edge from $u$ to $v$ means that $v$ cannot execute until $u$
finishes).  In this standard model, an edge typically has no weight (called
\defn{light-weight} edges).  In Muller and Acar's \defn{weighted dag} model,
if $v$ is a latency incurring operation (such as a blocking I/O), the latency
is modeled as an edge weight (called a \defn{heavy weight} edge). 

In the standard model, assuming unit-weight nodes, the \defn{work} $\work$ is
defined as the total number of nodes in the dag, or the time it takes to run
the computation on one core.  The \defn{span}\footnote{The term span is
sometimes called ``critical-path length'' and ``computation depth'' in the
literature.} ($\spa$) is defined as the length of a longest dependence chain
in the dag, or the time it takes to execute on infinitely-many cores.  Using
standard work stealing, a computation dag with work $\work$ and span $\spa$
can be executed on $P$ cores in expected time $\work / P + O(\spa)$.

In Muller and Acar's weighted dag model, the work is defined the same way
without the edge weight, since latency is not part of the computation, and the
span is defined as the length of a longest weighted dependence chain including
the edge weights.  Then, their scheduling algorithm can execute a computation
in time $O(\work / P + \spa \suspendWidth (1 + \lg \suspendWidth))$ in
expectation, where the $\suspendWidth$ is, effectively, the maximum number of
heavy-weight edges that cross a source-sink partition of the dag.
Intuitively, the $\suspendWidth$ correponds to the maximum number of latency
incurring operations that are logically in parallel.  Two things to note about
their bounds.  First, their algorithm is \defn{latency hiding}, since the
latency incurs no asymptotic overhead on the work term.  Second, if no latency
incurring operations are used, their algorithm results asymptotically the same
bound as the standard work stealing, $O(\work / P + \spa)$.  

% ============================================================

allow the worker to simply submit the I/O request asynchronously, and whenever
the result from the I/O must be obtained in order for the control to progress, 

%% ============================================================

Such I/O operations are typically done via low-level system libraries (e.g.,
the GNU C library) or through system calls provided by the Operating Systems
(OS).  Even though one could directly invoke functions provided by the
low-level system libraries within a task parallel program, doing so has
certain performance implications and/or can severely complicate the program
control flow.  Generally, two types of I/O operations are provided:
\defn{synchronous} I/O, where a call to perform I/O will block until the I/O
completes, or \defn{asynchronous} I/O, which is non-blocking, but handling the
I/O completion asynchronously can be complex.  

Directly invoking synchronous I/O operations can lead to performance
degradations.  Up on invoking a synchronous I/O operation, the \defn{worker
thread} --- surrogate of a processing core managed by the scheduler --- that
executes the I/O can potentially block for an extended period of time, leaving
one of the physical core underutilized.  One strategy to combat that is to
\defn{oversubscribe} the system, configuring the runtime to create many more
worker threads than the actual number of physical cores.  Doing so allows the
workers blocked on I/O to be context switched out with workers that have
actual comptuations to work on, thereby keeping the physical cores busy.
However, doing so has its own cost.  During the period when there is no I/O,
workers sharing a core can interfere with one another (e.g., competing on
private caches); during the period when there are blocking I/O operations, the
oversubscription strategy may not sufficiently combat the I/O latency effect
as the latency increases.  Finally, whether one oversubscribe the system or
not, such blocking invalidates the scheduling bound that the runtime could
otherwise provide.  

Submitting an asynchronous I/O request is simple, but handling the event
notification of I/O completion can be tricky.  One can configure the
notifcation to be delievered as a signal (e.g., Linux \texttt{aio}
facility~\cite{LinuxManPageAio19}), which requires the programmer to write
signal handling code that is challenging to get right, as the signal delivery
can occur at any point of execution (including when the worker is in the
scheduling code).  Another alternative is for the programmer to write explicit
polling code, checking back via the library API to see if the I/O has
completed (e.g., Linux \texttt{epoll} facility~\cite{LinuxManPageEpoll19}).
The periodic check via library API is simpler than handling signals, but
likely requires the programmer to rework the program control flow and can
incur additional overhead.  Finally, it is also possible to convert the signal
deliveries into callback events, and designate a separate persistent thread to
execute an event loop to handle all the callbacks (e.g., Linux
\texttt{libevent}~\cite{LinuxLibevent19}).  The last option is perhaps the
simplest.  However, it still requires the programmer to rework the task
parallel code to allow for synchronizations between the task parallel code and
the designated event-loop thread.  Moreover, since the synchronization is
performed by the user code outside of the scheduler's control, if the control
reaches a code point where the result from the I/O is necessary in order to
continue execution, we end up having the same issue of worker being blocked as
in the case of synchronous I/Os.  

%% ============================================================

In this paper, we study how to best incorporate I/O operations into a task
parallel platform.  It turns out that, the use of future constructs provides a
nice abstraction to allow the programmer to specify desired I/O operations and
enable the runtime to hide I/O latency.  Similar to fork-join parallelism, one
can \defn{spawn} off a \defn{future task} that executes logically in parallel
with the continuation of the spawn statement.  Unlike fork-join parallelism,
however, the termination of the future task is not constained to a particular
lexical scope.  Rather, the spawning of the future task returns a
\defn{handle}, which the programmer can later use to either query for the
status of the future task, or wait for its termination.  Since the handle (an
object in memory) can be passed around or stored in data structure and
retrieved later, it effectively promotes the associated future task into a
first-class object.  The use of futures is not new --- it has been proposed
since the late 70th~\cite{FriedmanWi78, BakerHe77} and its use has been
incorporated into various task parallel languages and
platforms~\cite{ChandraGuHe94, KranzHaMo89, Halstead85, CharlesGrSa05,
SpoonhowerBlHa08, FluetRaRe10, TasirlarSa11, CaveZhSh11, LuJiSc14}.
Nevertheless, we show how it can allow I/O operations to be nicely
incorporated into task parallel platforms 



